Derivative-Guided Symbolic Execution

We consider the formulation of a symbolic execution (SE) procedure for functional programs that interact with effectful, opaque libraries. Our procedure allows specifications of libraries and abstract data type (ADT) methods that are expressed in Linear Temporal Logic over Finite Traces (LTLf), interpreting them as symbolic finite automata (SFAs) to enable intelligent specification-guided path exploration in this setting. We apply our technique to facilitate the falsification of complex data structure safety properties in terms of effectful operations made by ADT methods on underlying opaque representation type(s). Specifications naturally characterize admissible traces of temporally-ordered events that ADT methods (and the library methods they depend upon) are allowed to perform. We show how to use these specifications to construct feasible symbolic input states for the corresponding methods, as well as how to encode safety properties in terms of this formalism. More importantly, we incorporate the notion of symbolic derivatives, a mechanism that allows the SE procedure to intelligently underapproximate the set of precondition states it needs to explore, based on the automata structures implicit in the provided specifications and the safety property that is to be falsified. Intuitively, derivatives enable symbolic execution to exploit temporal constraints defined by trace-based specifications to quickly prune unproductive paths and discover feasible error states. Experimental results on a wide-range of challenging ADT implementations demonstrate the effectiveness of our approach.

==> formalism.tex <==
\section{Formalism}

\subsection{Pure Symbolic Execution}

We begin by presenting the symbolic execution of purely functional
programs.  As the semantics of pure library functions is provided in
the form of refinement types, we convert them to \texttt{assert} and
\texttt{assume} expressions to facilitate symbolic
execution\todo{how}.

\begin{equation}
  \assertin{\phi}{e} \defeq \assumein{\phi}{e} ~\otimes~ \assumein{\neg\phi}{\abort}
\end{equation}

\begin{mathpar}
  \Infer{BugAbort}{
    \sat{\Phi} \\
  }{
    \left( \Phi, \abort \right) \hookrightarrow
    \left( \Phi, \bug \right)
  }

  \Infer{Assume}{}{
    \left( \Phi, \assumein{\phi}{e} \right) \hookrightarrow
    \left( \Phi \wedge \phi, e \right)
  }

  \Infer{ChoiceL}{}{
    \left( \Phi, e_1 \otimes e_2 \right) \hookrightarrow
    \left( \Phi, e_1 \right)
  }

  \Infer{ChoiceR}{}{
    \left( \Phi, e_1 \otimes e_2 \right) \hookrightarrow
    \left( \Phi, e_2 \right)
  }
\end{mathpar}

\begin{example}
  Let's check a pure function \inlinecaml{self_divide} against its
  refinement type.  Refinement type can be regarded as a form of
  specification where refinement on argument types denotes
  pre-condition and refinement on return type denotes post-condition.
  Therefore, we first introduce a symbolic variable for its argument
  \inlinecaml{x} and \inlinecaml{assume} that \inlinecaml{x} satisfies
  the pre-condition \inlinecaml{x > 0}.  Then before returning
  variable \inlinecaml{y}, we \inlinecaml{assert} that \inlinecaml{y}
  satisfies the post-condition \inlinecaml{y = 1}.
  Next, the refinement type
  \inlinecaml!x1:int -> x2:{v:int | x2 <> 0} -> {v:int | x1 / x2}!
  of \inlinecaml{divide} is converted accordingly; the pre-condition
  \inlinecaml!x <> 0! is enforced via \inlinecaml{assert} while the
  post-condition \inlinecaml!y = x / x! is \inlinecaml{assume}d to be
  true for the symbolic variable \inlinecaml!y! storing the result of
  \inlinecaml{divide}.  
  Now we explore all paths in the translated program (the middle one
  below) by collecting constraint $\Phi$ along each path.  Here are
  the constraint of the two paths leading to \inlinecaml{abort}:
  \begin{compactitem}
  \item \inlinecaml{$\Phi[1]$ = x > 0 $\wedge$ x = 0} and
  \item \inlinecaml{$\Phi[2]$ = x > 0 $\wedge$ x <> 0 $\wedge$ y = x / x $\wedge$ y != 1}
  \end{compactitem}
  As neither $\Phi[1]$ nor $\Phi[2]$ is satisfiable, we declare
  \inlinecaml{self_divide} to be safe against its refinement type.
  Had we assigned a weaker pre-condition \inlinecaml{x >= 0} to
  \inlinecaml{self_divide}, $\Phi[1]$ becomes satisfiable and the
  corresponding \inlinecaml{abort} becomes reachable.

  \hfill
  \begin{minipage}{.5\textwidth}
\begin{camlNoLines}
let divide x1 x2 =
  assert (x2 <> 0);
  let y = ?? in
  assume (y = x1 / x2); y
let self_divide x = divide x x
\end{camlNoLines}
  \end{minipage}%
  \begin{minipage}{.45\textwidth}
\begin{camlNoLines}
let run () =
  let x = ?? in
  assume (x > 0);
  let y = self_divide x in
  assert (y = 1)
\end{camlNoLines}
  \end{minipage}

  \qed
\end{example}
\todo[inline]{partial application? function
  argument?\cite{nguyenRelativelyCompleteCounterexamples2015}}


Then we introduce effectful function $\eff{f}$ calls.
Instead of tracking the symbolic state of libraries explicitly, we may
embed them in the history of effectful function calls and define the
semantics of effectful functions with respect to the histroy.
And the constraint on history is represented by symbolic finite
automata (SFA).  As a result, the refinement type of each effectful
functions needs to be augmented with SFA to capture its effectful
semantics.  Specifically, the return type is a disjuntion of different
refinements, each conditioned on an automaton $\FA$.
As an example, the return value of $\eff{get}~k$ for a key-value store
is given by the last $\eff{put}$ with key $k$.  \todo{expand}
Like refinements are converted to \texttt{assume}, we convert
automaton conditions to \texttt{admit}\todo{how}\todo{partial}.

\begin{align*}
  \letin{y}{\eff{f}~x}{e} \transeq 
  & \assertin{\toexp{x: t_x}}{} \\
  &\quad \left( \bigotimes_\idx \admitin{\FA[\idx]}{
      \assumein{\toexp{y : t_\idx}}{
        \appendin{\inangle{\eff{f}~x = y}}{e}}} \right) \\
  &\text{where}~ \eff{f}:g \dashrightarrow x:t_x \rightarrow \vert~ \wrap{\FA[\idx]}~ t_\idx
\end{align*}

\begin{example}
  Here is a simple effectful functional program that uses a key-value
  store.  The effect of the key-value store is captured using history
  of $\eff{put}$ and $\eff{get}$ calls.  For example,
  $\FA[store](k, v)$ denotes that key $k$ is bound to value $v$ in the
  store and $\FA[free](k)$ denotes that key $k$ is not bound in the
  store.
  \begin{align*}
    \FA[store](k, v) &\doteq~ \F \left(
                              \inangle{\eff{put}~k~v} \wedge
                              \X \neg \F \inangle{\eff{put}~k~\_} \right) \\
    \FA[free](k) &\doteq~ \neg \F \inangle{\eff{put}~k~\_} \\
  \end{align*}
  Unlike conventional symbolic execution, path condition is now
  augmented with symbolic automaton encoding the state of effecful
  libraries.  As a result, the satisfiability of such a path condition
  is equivalent to checking the non-emptiness of its automaton $\FA$
  under its propositional constraint $\Phi$.  For example, the
  \inlinecaml{abort} within \inlinecaml{assert} has the following path
  condition
  \begin{inparaenum}
  \item $\Phi[abort] = v \neq v'$ and
  \item $\FA[abort] = \inangle{\eff{put}~k~v} \wedge \F
    \inparen{\inangle{\eff{put}~k~v'} \wedge \X \neg \F
      \inangle{\eff{put}~k~\_}}$.
  \end{inparaenum}
  $\FA[abort]$ is empty under $\Phi[abort]$ despite $\Phi[abort]$
  itself is satisfiable.  Therefore, the path condition is not
  satisfiable and the bad case in \inlinecaml{assert} is not
  reachable.
  
  \begin{minipage}{.5\textwidth}\begin{center}\begin{tabular}{c}
\begin{camlNoLines}
let put k v = append <<put k v>>
let get k =
  let v = ?? in
  if * then
    admit(@$\FA[store](k, v)$@); v
  else
    admit(@$\FA[free](k)$@); abort
\end{camlNoLines}
  \end{tabular}\end{center}\end{minipage}%
  \begin{minipage}{.45\textwidth}\begin{center}\begin{tabular}{c}
\begin{camlNoLines}
let run () =
  let k = ?? in
  let v = ?? in
  put k v;
  let v' = get k in
  assert (v = v');
\end{camlNoLines}
  \end{tabular}\end{center}\end{minipage}
 
  \qed
\end{example}

\newpage
\begin{example}
  SFA can also express protocol about the usage of effectful
  libraries.  Imagine we want to enforce that $\eff{put}$ function
  calls always happen in order with relative to their keys.  We may
  impose this protocol on a simple client program that takes a boolean
  argument $b$ and returns unit value.  Its specification
  \[k_{1}:\var{key} \dasharrow k_{2}:\{v:\var{key}\mid k_{1} < v\} \dasharrow b:\var{bool} \rightarrow \wrap{\varepsilon} \var{unit} \wrap{\FA[order](k_{1}, k_{2})}\]
  states that for all ordered pairs of keys $k_{1}$ and $k_{2}$, all
  traces of effectful function calls made in the client program are
  accepted by $\FA[order](k_{1}, k_{2})$.
  And $\FA[order](k_{1}, k_{2})$ affirms that any $\eff{put}$ with the
  larger key $k_{2}$ can only happen after the $\eff{put}$ with the
  smaller key $k_{1}$ for all emitted traces.
  \begin{align*}
    \FA[order](k_1, k_2) \doteq~ & \neg\inangle{\eff{put}~k_2~\_} ~\W~ \inangle{\eff{put}~k_1~\_} \\
    \doteq~                      & (\bullet / \inangle{\eff{put}~k_2~\_})^* \vee
                                   \inparen{(\bullet / \inangle{\eff{put}~k_2~\_})^* ~ \inangle{\eff{put}~k_1~\_} ~ \bullet^*} 
  \end{align*}
\begin{camlNoLines}[numbers=left]
let run () =
  let g1, g2 = ??, ?? in
  assume g1 < g2;
  let b = ?? in
  put 2 2;
  if b then put 3 3
  else put 1 1
  affirm (@$\FA[order](g1, g2)$@)
\end{camlNoLines}
  \begin{enumerate}
  \item Taking the first branch of \inlinecaml{if}, the path condition
    at \inlinecaml{abort} consists of $\Phi[1] = (g_1 < g_2) \wedge b$
    and
    $\FA[1] = \inangle{\eff{put}~2~2} \inangle{\eff{put}~3~3} \wedge \neg \FA[order](g_1, g_2)$.
    As our goal is to find \emph{any} assignment to $g_{1}$
    and $g_{2}$ that makes $\Phi[1]$ satisfiable and $\FA[1]$ is
    non-empty, $\neg\FA[order](g_{1}, g_{2})$ denotes all traces with
    a pair of $\eff{put}$ with decreasing keys.  Conjoined with a pair
    of $\eff{put}$ with increasing keys, $\FA[1]$ is deemed empty
    regardless of the satisfiable assignment to $g_{1}$ and $g_{2}$.
    \inlinecaml{abort} is not reachable from the first \inlinecaml{if}
    branch.

  \item Taking the second branch of \inlinecaml{if}, the path
    condition at \inlinecaml{abort} consists
    of $\Phi[2] = (g_1 < g_2) \wedge \neg b$
    and
    $\FA[2] = \inangle{\eff{put}~2~2} \inangle{\eff{put}~1~1} \wedge \neg \FA[order](g_1, g_2)$.
    As $\neg\FA[order](g_{1}, g_{2})$ is now conjoined with a pair of
    decreasing keys, $2$ and $1$.  We have such a satisfiable
    assignment $g_{1} = 2 \wedge g_{2} = 1$ that $\FA[2]$ accepts
    trace $\inangle{\eff{put}~2~2} \inangle{\eff{put}~1~1}$.
  \end{enumerate}
\qed  
\end{example}

The non-emptiness of $\FA[1]$ and $\FA[2]$ may not be too hard for a
``smart'' solver to check since both have a concrete trace as one of
their conjuncts.  In practice, pre-condition SFA of all library
function calls along a path needs to be conjoined to the negation of
the SFA specifying the protocol.  For example, $\eff{get}~k$ requires
the current trace to be accepted by $\FA[store](k, v)$ for some $v$
while $\eff{put}$ has no requirement for the current trace.
Before checking the emptiness of conjoined SFAs - unlike
satisfiability check of propositional formula - we (or the solver)
have to \emph{compute} their intersection, which may drastically
increase the number of states in the resulting automata.  Therefore,
simply augmenting path condition with SFAs would greatly degrade the
scalability of symbolic execution.



\begin{mathpar}
  \Infer{Sat}{
    \sigma \in \denot{\Phi} \\
    \pi \in \lang(\sigma(\FA))
  }{
    \sat{\Phi, \FA}
  }

  \Infer{BugAbort}{
    \sat{\Phi, \FA}
  }{
    \left( \Phi, \FA, \abort \right) \hookrightarrow
    \left( \Phi, \FA, \bug \right)
  }

  \Infer{Admit}{}{
    \left( \Phi, \FA, \admitin{\FA'}{e} \right) \hookrightarrow
    \left( \Phi, \FA \wedge \FA', e \right)
  }

  \Infer{Append}{}{
    \left( \Phi, \FA, \appendin{\inangle{\eff{f}~x = y}}{e} \right) \xhookrightarrow{\inangle{\eff{f}~x = y}}
    \left( \Phi, ~\FA ; \inangle{\eff{f}~x = y}~, e \right)
  }

  \Infer{FANotSub}{
    \sigma \in \denot{\Phi} \\
    \trace[curr] \in \lang(\sigma(\FA[0])) \\
    \trace \in \lang(\sigma(\FA[1])) \\
    \trace \notin \lang(\sigma(\FA[2]))
  }{
    \Phi, \FA[0] \vdash \FA[1] \not\subseteq \FA[2]
  }

  \Infer{Refute}{
    \left( \Phi, \FA[curr], e \right) \xhookrightarrow{\Trace}\!\!^* \left(\Phi', \FA[curr]', v \right) \\
    \Phi', \FA[curr]' \vdash \Trace \not\subseteq \FA \\
  }{
    \left( \Phi, \FA[curr], \FA, e\right) : \bot
  }
\end{mathpar}



We then leverage automata derivatives to refute program at the
earliest point possible. We inherit \textsc{Sat}, \textsc{Bug}, and
\textsc{Admit} from last set of rules by simply passing the additional
$\FA[cont]$ through.

\begin{mathpar}
  \Infer{BugEmptyFA}{
    \sigma \in \denot{\Phi} \\
    \pi \in \lang(\sigma(\FA[curr])) \\
    \lang(\sigma(\FA[cont])) \equiv \varnothing \\
  }{
    \left(\Phi, \FA[curr], \FA[cont], e\right) \hookrightarrow
    \left(\Phi, \FA[curr], \FA[cont], \bug\right)
  }

  \Infer{BugNonNullableFA}{
    \sat{\Phi, \FA[curr]} \\
    \isnullableFA{\FA[cont]} \\
  }{
    \left(\Phi, \FA[curr], \FA[cont], v\right) \hookrightarrow \left(\Phi, \FA[curr], \FA[cont], \bug\right)
  }

  \Infer{Append}{
    \FA[curr]' = \FA[curr]; \inangle{\eff{f}~x = y} \\
    \left(\Phi, \FA[cont]\right) \xrightharpoonup{\inangle{\eff{f}~x = y}} \left(\Phi', \FA[cont]'\right) \\
  }{
    \left(\Phi, \FA[curr], \FA[cont], \appendin{\inangle{\eff{f}~x = y}}{e}\right) \hookrightarrow
    \left(\Phi', \FA[curr]', \FA[cont]', e\right)
  }

  \Infer{Refute}{
    \left(\Phi, \FA[curr], \FA[cont], e\right) \hookrightarrow\!\!^* \left(\Phi', \FA[curr]', \FA[cont]', \bug\right) \\
  }{
    \left(\Phi, \FA[curr], \FA[cont], e\right) : \bot
  }
\end{mathpar}

One way to improve the scalability is leverage the regularity of
automata - we may examine one symbol at a time to determine if a word
is accepted by a automata\todo{expand}.  Notice that instead of SFA
emptiness checking, we may check if all emitted trace can be accepted
by the protocol SFA.

\begin{example}
  Consider the same example as above.  The first function call can be
  be $\inangle{\eff{put}~k_{1}~\_}$ or $!\inangle{\eff{put}~k_{2}~\_}$.  We branch the execution by
  adding $k_{1} = 2$ and $k_{1} \neq 2$ to the respective path
  condition.
  \[ \partial_{\inangle{\eff{put}~2~2}} \FA[order] \]
\end{example}

\begin{example}
  slightly more complex
\begin{camlNoLines}[numbers=left]
let run () =
  let g1, g2 = ??, ?? in
  assume g1 < g2;
  let k = ??;
  put k 2;
  if k < 2 then put 3 3
  else put 1 1
  affirm (@$\FA[order](g1, g2)$@)
\end{camlNoLines}
\end{example}

\begin{example}
  Even with derivative computation, we still need to check the
  emptiness of symbolic automaton for each execution path.

  \begin{align*}
    \FA[nxt](m, n) \doteq & \F \left(
                       \inangle{\mathtt{setNxt}~m~n} \wedge
                       \X \neg \F \inangle{\mathtt{setNxt}~m~\_} \right) \\
    \FA[val](n, v) \doteq & \F \left(
                       \inangle{\mathtt{setVal}~n~v} \wedge
                       \X \neg \F \inangle{\mathtt{setVal}~n~\_} \right) \\
  \end{align*}

  \begin{enumerate}
  \item \cref{line:remove:hd-null}:
    $\Phi \doteq hd_0 = \var{null}$ and
    $\FA[curr] \doteq \FA[nxt](m, n)$
  \item \cref{line:remove:hd-v}:
    $\Phi \doteq hd_0 \neq \var{null} \wedge v = v_0$,
    $\FA[curr] \doteq
    \FA[nxt](m, n) \wedge \FA[val](hd_0, v_0) \wedge \FA[nxt](hd_0,
    hd_1)$, and
    $\Trace = \varepsilon$
  \item \cref{line:remove:end}:
    $\Phi \doteq
    hd_0 \neq \var{null} \wedge v_0 \neq v \wedge hd_1 = \var{null}$,
    $\FA[curr] \doteq
    \FA[nxt](m, n) \wedge \FA[val](hd_0, v_0) \wedge \FA[nxt](hd_0,
    hd_1)$, and
    $\Trace = \varepsilon$
  \item \cref{line:remove:set-next}:
    $\Phi \doteq
    hd_0 \neq \var{null} \wedge v_0 \neq v \wedge hd_1 \neq \var{null} \wedge v_1 = v$,
    $\FA[curr] \doteq
    \FA[nxt](m, n) \wedge \FA[val](hd_0, v_0) \wedge \FA[nxt](hd_0,
    hd_1) \wedge \FA[val](hd_1, v_1) \wedge \FA[nxt](hd_1, hd_2)$, and
    $\Trace = \inangle{\mathtt{setNxt}~hd_0~hd_2}$
  \end{enumerate}
  
  To further improve the scalability
  of symbolic execution,
  we start symbolic execution with trace being a constant repetition
  of \inlinecaml{.} event instead of \inlinecaml{.*}.  This allows
  \inlinecaml{admit} to refine the symbolic trace instead of
  conjugating all automaton along each execution path.  The refinement
  also emits propositional constraints on (ghost) variables in the
  context.

  \begin{minipage}{.52\textwidth}
\begin{camlNoLines}[numbers=left]
let remove hd v =
  if hd = null then hd(@\label{line:remove:hd-null}@)
  else if get_value hd = v then
    get_next hd(@\label{line:remove:hd-v}@)
  else
    let rec loop curr =
      let next = get_next curr in
      if next = null then ()(@\label{line:remove:end}@)
      else if get_value next = v then
        (@@)``set_next curr (get_next next)``(@\label{line:remove:set-next}@)
      else loop next
    in loop hd; hd
\end{camlNoLines}
  \end{minipage}%
  \begin{minipage}{.45\textwidth}
\begin{camlNoLines}
let run () =
  let g_a, g_b = ??, ?? in
  admit F (<<set_next g_a g_b>> &&
        X G !<<set_next g_a _>>);
  let hd0, v = ??, ?? in
  label st;
  let hd = remove hd0 v in
  affirm(@@)@st !<<set_next _ g_b>>
            W <<set_next g_a _>>
\end{camlNoLines}
  \end{minipage}

  \qed
\end{example}

Noticing while Rule FAEmpty allows us to find potential bugs at any
program point, its premise is generally undecidable.

\paragraph{Boolean Event Algebra}
Symbolic events in event literals are associated with disjoint functions.
\[\arraycolsep=4pt
  \begin{array}{llrl}
    \text{Symbolic Event} & \alpha, \beta & ::= & \inangle{\eff{f}} \mid \inangle{\eff{f}~\overline{x} = y} \\
    \text{Event Literal}  & \literal      & ::= & \left(\alpha_1 \parallel \dots \parallel \alpha_k \right) \\
    \text{Event Sequence} & \Trace        & ::= & [] \mid \literal :: \Trace 
  \end{array}
\]

\todo[inline]{definition of boolean operations}

\begin{mathpar}
  \Infer{BugAbort}{
    \sat{\Phi}
  }{
    \left( \Phi, \Pi, \FA, \abort \right) \hookrightarrow
    \left( \Phi, \Pi, \FA, \bug \right)
  }

  \hva \and

  \Infer{Bug-$\varepsilon$}{
    \sat{\Phi} \\
    \neg\isnullableFA{\FA} \\
  }{
    \left(\Phi, \Trace, \FA, v\right) \hookrightarrow \left(\Phi, \Trace, \FA, \bug\right)
  }

  \Infer{Bug-$\varnothing$}{
    \sigma \in \denot{\Phi}\\
    \lang(\sigma(\FA)) \equiv \varnothing \\
  }{
    \left(\Phi, \Trace, \FA, e\right) \hookrightarrow
    \left(\Phi, \Trace, \FA, \bug\right)
  }

  \Infer{Admit}{
    \left(\Phi, \Pi, \FA\right)
    \xrightharpoonup{\overline{g}}
    \left(\Phi', \Pi', \FA'\right) \\
    \sat{\Phi'} \\
    \isnullableFA{\FA'} \\
  }{
    \left( \Phi, \Pi, \FA[cont], \admitin[\overline{g}]{\FA}{e} \right) \hookrightarrow
    \left( \Phi', \Pi', \FA[cont], e \right)
  }

  \Infer{Append}{
    \left(\Phi, \inangle{\eff{f}~x = y}, \FA\right) \rightharpoonup
    \left(\Phi', \literal, \FA'\right) \\
  }{
    \left(\Phi, \Trace, \FA, \appendin{\inangle{\eff{f}~x = y}}{e}\right) \hookrightarrow
    \left(\Phi', \Trace \doubleplus [\literal], \FA', e\right)
  }

  \Infer{Refute}{
    \left(\Phi, \FA[curr]\right) \rightsquigarrow \left(\Phi', \Trace\right) \\
    \left(\Phi', \Trace, \FA[cont], e\right) \hookrightarrow\!\!^* \left(\Phi'', \Trace', \FA[cont]', \bug\right) \\
  }{
    \left(\Phi, \FA[curr], \FA[cont] , e\right) : \bot
  }
\end{mathpar}

\begin{mathpar}
  \Infer{Sample}{
    \left( \Psi, \literal \right) \in \FAnext(\FA) \\
    \Phi' = \Phi \wedge \Psi \\
    \sat{\Phi'} \\
    \left(\Phi', \partial_\literal^{\Phi'} \FA \right) \rightsquigarrow \left(\Phi'', \Trace\right) \\
  }{
    \left(\Phi, \FA\right) \rightsquigarrow \left(\Phi'', \literal :: \Trace\right)
  }

  \Infer{Deriv}{
    \left(\Psi, \literal'\right) \in \FAnext(\literal) \ltimes \FAnext(\FA) \\
    \Phi' = \Phi \wedge \Psi \\
    \sat{\Phi'} \\
  }{
    \left(\Phi, \literal, \FA\right)
    \rightharpoonup
    \left(\Phi', \literal', \partial_{\literal'}^{\Phi'} \FA\right)
  }

  \Infer{Deriv-$\exists$}{
    (\literal', \FA') \in \FAuncons_{\overline{g}}^{\Phi} (\FA) \\
    \literal \sqcap \literal' = \Psi, \literal'' \\
  }{
    \left(\Phi, \literal, \FA\right)
    \xrightharpoonup{\overline{g}}
    \left(\Phi \wedge \Psi, \literal'', \FA'\right)
  }

  \Infer{DerivBase-$\exists$}{}{
    (\Phi, [], \FA)
    \xrightharpoonup{\overline{g}}
    (\Phi, [], \FA)
  }

  \Infer{DerivInd-$\exists$}{
    (\Phi, \literal, \FA) \xrightharpoonup{\overline{g}} (\Phi', \literal', \FA') \\
    (\Phi', \Pi, \FA') \xrightharpoonup{\overline{g}} (\Phi'', \Pi', \FA'')
  }{
    \left(\Phi, \literal {::} \Pi, \FA\right)
    \xrightharpoonup{\overline{g}}
    \left(\Phi'', \literal' {::} \Pi', \FA''\right)
  }
\end{mathpar}






Now let's introduce existentially quantified automata.
\begin{example}
  Consider effectful function
  $\eff{get} : c: \type{value} \dashrightarrow k: \type{key}
  \rightarrow \wrap{\FA} \{ v: \type{value} \mid v = c \}$, where
  $\FA = \bullet^*; \inangle{\eff{put}~\var{k}~\var{v} \mid \var{k} = k \wedge \var{v} = v}; \inangle{\eff{put}~\var{k}~\var{v} \mid \var{k} = k}^\complement$.
  We call $\eff{get}$ on local variable $k$ under symbolic state $(x > 0, [\inangle{\eff{put}~\var{k}~\var{v} \mid \var{k} = k \wedge
    \var{v} > x}])$.
  Then $\left(\Phi, \alpha, \FA\right)
  \stackrel{v}{\blacktriangleright}_\idx
  \left(\Phi \wedge \Psi, \alpha', \FA'\right)$, where
  \begin{enumerate}
  \item  $\alpha' = $, $\Psi = \inparen{\var{k}_\idx = k \wedge \var{v}_\idx > x \wedge \var{v}_\idx = v}$,
  \end{enumerate}
\end{example}

\begin{equation}
  \FAuncons^{\overline{a}}_{\Phi} (\FA) = \left\{
    (\alpha, \partial_\alpha^{\overline{a}} \FA) \mid \alpha \in \FAnext^{\overline{a}}_{\Phi} (\FA) 
  \right\}
\end{equation}


\begin{mathpar}
  \todo[inline]{other cases of anti-unification}


\end{mathpar}













